LoRC: Low-Rank Compression for LLMs KV Cache with a Progressive Compression Strategy

The Key-Value (KV) cache is a crucial component in serving transformer-based autoregressive large language models (LLMs), enabling faster inference by storing previously computed KV vectors. However, its memory consumption scales linearly with sequence length and batch size, posing a significant bottleneck in LLM deployment. Existing approaches to mitigate this issue include: (1) efficient attention variants integrated in upcycling stages, which requires extensive parameter tuning thus unsuitable for pre-trained LLMs; (2) KV cache compression at test time, primarily through token eviction policies, which often overlook inter-layer dependencies and can be task-specific. This paper introduces an orthogonal approach to KV cache compression. We propose a low-rank approximation of KV weight matrices, allowing for plug-in integration with existing transformer-based LLMs without model retraining. To effectively compress KV cache at the weight level, we adjust for layerwise sensitivity and introduce a progressive compression strategy, which is supported by our theoretical analysis on how compression errors accumulate in deep networks. Our method is designed to function without model tuning in upcycling stages or task-specific profiling in test stages. Extensive experiments with LLaMA models ranging from 8B to 70B parameters across various tasks show that our approach significantly reduces the GPU memory footprint while maintaining performance.

==> checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and precede the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The claims made in the abstract and introduction are supported by our experiments.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We discuss the limitations in Appendix.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not include theoretical results. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have provided the core code. The entire repository will be open-sourced later.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We currently provide the main model file to elaborate our method and reproducing. We will release all the model and code in the future.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our method focuses on the inference of LLMs, which does not require training, so there is no training details. For testing, we will provide the code for reproducing.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our experiments are inference-only tasks.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Provided in Appnedix.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: They are properly credited.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification:  We currently provide the main model file to elaborate our method and reproducing. We will release all the model and code in the future.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

==> theory_analysis.tex <==
\section{Error Bounds for KV Cache Compression}

In this section, we derive tight error bounds for the KV cache compression method, considering both individual layer errors and their propagation through a deep network.

\subsection*{Theorem 1: Single Layer Error Bound}

Let \( W \in \mathbb{R}^{m \times n} \) be a weight matrix (either key or value), and let \( W_k \in \mathbb{R}^{m \times n} \) be its rank-\( k \) approximation obtained via truncated singular value decomposition (SVD). For any input vector \( x \in \mathbb{R}^n \), the error introduced by the approximation is bounded by:
\begin{equation}
\| W x - W_k x \|_2 \leq \sigma_{k+1} \| x \|_2,
\end{equation}
where \( \sigma_{k+1} \) is the \( (k+1) \)-th singular value of \( W \).

\textbf{Proof.}

Let \( W = U \Sigma V^\top \) be the full SVD of \( W \), where \( U \in \mathbb{R}^{m \times m} \) and \( V \in \mathbb{R}^{n \times n} \) are orthogonal matrices, and \( \Sigma = \operatorname{diag}(\sigma_1, \ldots, \sigma_n) \) with singular values \( \sigma_1 \geq \sigma_2 \geq \cdots \geq \sigma_n \geq 0 \).

The rank-\( k \) approximation \( W_k \) is given by:
\[
W_k = U_k \Sigma_k V_k^\top,
\]
where \( U_k \), \( \Sigma_k \), and \( V_k \) are truncated versions of \( U \), \( \Sigma \), and \( V \), respectively, keeping only the first \( k \) singular values and corresponding vectors.

We have:
\begin{align*}
\| W x - W_k x \|_2 &= \| (W - W_k) x \|_2 \\
&= \| U (\Sigma - \Sigma_k) V^\top x \|_2 \\
&= \| \operatorname{diag}(0, \ldots, 0, \sigma_{k+1}, \ldots, \sigma_n) V^\top x \|_2,
\end{align*}
since \( U \) is orthogonal and preserves the \( \ell_2 \)-norm.

From this expression, we obtain:
\begin{align*}
\| W x - W_k x \|_2 &\leq \sigma_{k+1} \| V^\top x \|_2 \\
&= \sigma_{k+1} \| x \|_2,
\end{align*}
as \( V \) is also orthogonal.

\hfill \(\square\)

\subsection*{Theorem 2: Error Propagation Bound}

Consider an \( L \)-layer network where each layer \( i \) applies a linear transformation \( W_i \) followed by a 1-Lipschitz nonlinearity \( \phi \) (e.g., ReLU, tanh). Let \( \tilde{W}_i \) be the compressed version of \( W_i \) obtained via truncated SVD with rank \( k_i \). The error at the output of the network is bounded by:
\begin{equation}
\| x_L - \tilde{x}_L \|_2 \leq \sum_{i=1}^L \left( \sigma_{k_i+1}^{(i)} \prod_{j=i+1}^L \| W_j \|_2 \right),
\end{equation}
where \( x_L \) and \( \tilde{x}_L \) are the outputs of the original and compressed networks, respectively; \( \sigma_{k_i+1}^{(i)} \) is the \( (k_i+1) \)-th singular value of \( W_i \); and \( \| W_j \|_2 \) denotes the spectral norm of \( W_j \).

\textbf{Proof.}

Let \( x_i \) and \( \tilde{x}_i \) denote the outputs of the \( i \)-th layer in the original and compressed networks, respectively. We prove by induction that:
\begin{equation}
\| x_i - \tilde{x}_i \|_2 \leq \sum_{s=1}^i \left( \sigma_{k_s+1}^{(s)} \prod_{j=s+1}^i \| W_j \|_2 \right).
\end{equation}

\textbf{Base Case (\( i = 1 \)).}

Using Theorem 1 and the 1-Lipschitz property of \( \phi \):
\begin{align*}
\| x_1 - \tilde{x}_1 \|_2 &= \| \phi(W_1 x_0) - \phi(\tilde{W}_1 x_0) \|_2 \\
&\leq \| W_1 x_0 - \tilde{W}_1 x_0 \|_2 \\
&\leq \sigma_{k_1+1}^{(1)} \| x_0 \|_2.
\end{align*}

\textbf{Inductive Step.}

Assume the inductive bound holds for layer \( i-1 \). For layer \( i \):
\begin{align*}
\| x_i - \tilde{x_i} \|_2 &= \| \phi(W_i x_{i-1}) - \phi(\tilde{W}_i \tilde{x}_{i-1}) \|_2 \\
&\leq \| W_i x_{i-1} - \tilde{W}_i \tilde{x}_{i-1} \|_2 \\
&\leq \| W_i \|_2 \| x_{i-1} - \tilde{x}_{i-1} \|_2 + \sigma_{k_i+1}^{(i)} \| \tilde{x}_{i-1} \|_2,
\end{align*}
where the last inequality follows from Theorem 1 and the sub-multiplicative property of the spectral norm.

For simplicity, we overestimate \( \| W_i \|_2 + \sigma_{k_i+1}^{(i)} \leq 2 \| W_i \|_2 \) (assuming \( \sigma_{k_i+1}^{(i)} \leq \| W_i \|_2 \)):
\begin{equation}
\| x_i - \tilde{x}_i \|_2 \leq \sum_{s=1}^i \left( \sigma_{k_s+1}^{(s)} \prod_{j=s+1}^i 2 \| W_j \|_2 \right),
\end{equation}
which confirms the inductive bound holds for \( i \).

At the output layer (\( i = L \)), we have:
\[
\| x_L - \tilde{x}_L \|_2 \leq \sum_{i=1}^L \left( \sigma_{k_i+1}^{(i)} \prod_{j=i+1}^L 2 \| W_j \|_2 \right).
\]

\hfill \(\square\)

\subsection*{Corollary: Bound on Performance Degradation}

Let \( f(x) \) be the output of the original network and \( \tilde{f}(x) \) be the output of the compressed network for input \( x \). Assume the loss function \( \mathcal{L} \) is \( L_{\mathcal{L}} \)-Lipschitz in its first argument. The performance degradation is bounded by:
\begin{equation}
| \mathcal{L}(f(x), y) - \mathcal{L}(\tilde{f}(x), y) | \leq L_{\mathcal{L}} \| x_L - \tilde{x}_L \|_2 \leq L_{\mathcal{L}} \sum_{i=1}^L \left( \sigma_{k_i+1}^{(i)} \prod_{j=i+1}^L 2 \| W_j \|_2 \right),
\end{equation}
where \( y \) is the true label.

\textbf{Proof.}

Since \( \mathcal{L} \) is \( L_{\mathcal{L}} \)-Lipschitz in its first argument:
\[
| \mathcal{L}(f(x), y) - \mathcal{L}(\tilde{f}(x), y) | \leq L_{\mathcal{L}} \| f(x) - \tilde{f}(x) \|_2 = L_{\mathcal{L}} \| x_L - \tilde{x}_L \|_2.
\]
Substituting the bound from Theorem 2 completes the proof.

\hfill \(\square\)



\section{Information-Theoretic Analysis of KV Cache Compression}

In this section, we analyze the KV cache compression method from an information-theoretic perspective, focusing on the trade-off between compression ratio and information preservation.

\subsection{Preliminaries}

Let \( X \in \mathbb{R}^n \) be a random vector representing the input to a layer, and let \( W \in \mathbb{R}^{m \times n} \) be the weight matrix of the layer. The output of the layer is given by:
\begin{equation}
\label{eq:layer_output}
Y = W X.
\end{equation}

We compress \( W \) by approximating it with its rank-\( k \) truncated singular value decomposition (SVD), denoted by \( W_k \). The compressed output is then:
\begin{equation}
\label{eq:compressed_output}
\tilde{Y} = W_k X.
\end{equation}

\subsection{Variance Preservation}

Assuming that \( X \) is a zero-mean random vector with covariance matrix \( \Sigma_X \), the covariance matrices of \( Y \) and \( \tilde{Y} \) are:
\begin{align}
\Sigma_Y &= W \Sigma_X W^\top, \label{eq:cov_Y} \\
\tilde{\Sigma}_Y &= W_k \Sigma_X W_k^\top. \label{eq:cov_tildeY}
\end{align}

When \( \Sigma_X = I \) (i.e., \( X \) has identity covariance), these simplify to:
\begin{align}
\Sigma_Y &= W W^\top, \label{eq:cov_Y_identity} \\
\tilde{\Sigma}_Y &= W_k W_k^\top. \label{eq:cov_tildeY_identity}
\end{align}

Let \( \sigma_1 \geq \sigma_2 \geq \dots \geq \sigma_n \geq 0 \) be the singular values of \( W \). Then, the total variance of the outputs is:
\begin{align}
\operatorname{tr}(\Sigma_Y) &= \sum_{i=1}^n \sigma_i^2, \label{eq:total_variance_Y} \\
\operatorname{tr}(\tilde{\Sigma}_Y) &= \sum_{i=1}^k \sigma_i^2. \label{eq:total_variance_tildeY}
\end{align}

The fraction of the total variance preserved by the compression is:
\begin{equation}
\label{eq:variance_fraction}
\gamma = \frac{\operatorname{tr}(\tilde{\Sigma}_Y)}{\operatorname{tr}(\Sigma_Y)} = \frac{\sum_{i=1}^k \sigma_i^2}{\sum_{i=1}^n \sigma_i^2}.
\end{equation}

\subsection{Information Preservation}

Assuming that both \( X \) and \( Y \) are Gaussian random vectors, the differential entropy of \( Y \) is:
\begin{equation}
\label{eq:entropy_Y}
H(Y) = \frac{1}{2} \ln\left( (2\pi e)^m |\Sigma_Y| \right).
\end{equation}

Similarly, for \( \tilde{Y} \):
\begin{equation}
\label{eq:entropy_tildeY}
H(\tilde{Y}) = \frac{1}{2} \ln\left( (2\pi e)^m |\tilde{\Sigma}_Y| \right).
\end{equation}

To handle the singularity of \( \tilde{\Sigma}_Y \), we introduce a small additive isotropic noise \( \epsilon I \) to the covariance matrices:
\begin{align}
\Sigma_Y^\epsilon &= \Sigma_Y + \epsilon I, \label{eq:regularized_cov_Y} \\
\tilde{\Sigma}_Y^\epsilon &= \tilde{\Sigma_Y} + \epsilon I. \label{eq:regularized_cov_tildeY}
\end{align}

The mutual information between \( X \) and \( Y \) is:
\begin{equation}
\label{eq:mutual_information}
I(X;Y) = H(Y) - H(Y|X).
\end{equation}

Since \( Y \) is a deterministic linear transformation of \( X \), \( H(Y|X) = 0 \), and thus \( I(X;Y) = H(Y) \). Similarly for \( \tilde{Y} \).

The difference in mutual information due to compression is:
\begin{equation}
\label{eq:mutual_information_difference}
\Delta I = I(X;Y) - I(X;\tilde{Y}) = H(Y) - H(\tilde{Y}).
\end{equation}

Using the regularized covariance matrices, we have:
\begin{align}
H(Y) &= \frac{1}{2} \ln\left( (2\pi e)^m |\Sigma_Y^\epsilon| \right), \label{eq:entropy_Y_regularized} \\
H(\tilde{Y}) &= \frac{1}{2} \ln\left( (2\pi e)^m |\tilde{\Sigma}_Y^\epsilon| \right). \label{eq:entropy_tildeY_regularized}
\end{align}

\subsection{Theorem: Fraction of Information Preserved}

\textbf{Statement.} Compressing \( W \) to its rank-\( k \) approximation \( W_k \) via truncated SVD preserves at least a fraction \( \gamma \) of the output variance and approximately preserves a fraction \( \gamma \) of the information, where:
\begin{equation}
\label{eq:gamma_definition}
\gamma = \frac{\sum_{i=1}^k \sigma_i^2}{\sum_{i=1}^n \sigma_i^2}.
\end{equation}

\textbf{Proof.}

From \eqref{eq:variance_fraction}, we have shown that \( \gamma \) represents the fraction of variance preserved. Assuming that the information content is related to the variance captured (which holds for Gaussian distributions), the fraction of information preserved is approximately \( \gamma \).

\hfill \(\square\)

\subsection{Practical Guideline: Choosing the Compression Rank}

Given a desired information preservation ratio \( \alpha \) (e.g., \( 95\% \)), the optimal compression rank \( k^\ast \) can be determined by:
\begin{equation}
\label{eq:optimal_k}
k^\ast = \min \left\{ k : \frac{\sum_{i=1}^k \sigma_i^2}{\sum_{i=1}^n \sigma_i^2} \geq \alpha \right\}.
\end{equation}

This guideline provides a direct method to select the appropriate rank \( k \) that balances compression efficiency with information retention.


==> theory_generalization.tex <==
Here's the LaTeX version of your section on "Generalization Bounds Analysis for Compressed Models":

```latex
\section{Generalization Bounds Analysis for Compressed Models}

In this section, we derive generalization bounds for compressed neural network models using techniques from statistical learning theory, specifically leveraging PAC-Bayesian theory and matrix concentration inequalities. Our goal is to understand how model compression, particularly through low-rank approximations of weight matrices, affects the generalization performance of neural networks.

\subsection{Preliminaries}

Let us define the following:

\begin{itemize}
    \item \( \mathcal{H} \): the hypothesis space of the original (uncompressed) model.
    \item \( \mathcal{H}_c \): the hypothesis space of the compressed model, obtained by applying compression techniques to the weight matrices.
    \item \( L_D(h) \): the true risk (expected loss) of hypothesis \( h \) with respect to the data distribution \( D \).
    \item \( L_S(h) \): the empirical risk of hypothesis \( h \) on a sample \( S \) of size \( n \).
    \item \( n \): the number of samples in \( S \).
    \item \( d_i \): the dimension of the weight matrix \( W_i \) in layer \( i \).
    \item \( k_i \): the rank of the compressed weight matrix \( W_{k_i} \) in layer \( i \).
    \item \( \sigma_{k_i+1}^{(i)} \): the \( (k_i + 1) \)-th singular value of \( W_i \).
\end{itemize}

We consider loss functions that are bounded in \([0, 1]\) for normalization.

\subsection{Theorem 1: PAC-Bayesian Generalization Bound}

\textbf{Theorem 1.} For any prior distribution \( P \) over \( \mathcal{H}_c \), any \( \delta \in (0, 1) \), and any posterior distribution \( Q \) over \( \mathcal{H}_c \), with probability at least \( 1 - \delta \) over the choice of an i.i.d. sample \( S \) of size \( n \), the following inequality holds:
\begin{equation}
\label{eq:pac_bayes_bound}
L_D(Q) \leq L_S(Q) + \sqrt{\frac{\mathrm{KL}(Q \| P) + \ln\left(\frac{2\sqrt{n}}{\delta}\right)}{2n}},
\end{equation}
where \( L_D(Q) = \mathbb{E}_{h \sim Q}[L_D(h)] \), \( L_S(Q) = \mathbb{E}_{h \sim Q}[L_S(h)] \), and \( \mathrm{KL}(Q \| P) \) is the Kullback-Leibler divergence between \( Q \) and \( P \).

\textbf{Proof.}

We start from the classical PAC-Bayesian theorem \citep{catoni2007pac}, which states that for any \( \delta \in (0, 1) \), with probability at least \( 1 - \delta \):
\begin{equation}
\label{eq:pac_bayes_kl}
\mathrm{KL}\big(L_S(Q) \big\| L_D(Q)\big) \leq \frac{\mathrm{KL}(Q \| P) + \ln\left(\frac{2\sqrt{n}}{\delta}\right)}{n},
\end{equation}
where \( \mathrm{KL}(a \| b) \) denotes the Kullback-Leibler divergence between Bernoulli distributions with parameters \( a \) and \( b \).

Since the KL divergence between Bernoulli variables satisfies \( \mathrm{KL}(a \| b) \geq 2(a - b)^2 \) for \( a, b \in [0, 1] \), we have:
\begin{equation}
\label{eq:kl_lower_bound}
\mathrm{KL}\big(L_S(Q) \big\| L_D(Q)\big) \geq 2\left(L_S(Q) - L_D(Q)\right)^2.
\end{equation}

Combining \eqref{eq:pac_bayes_kl} and \eqref{eq:kl_lower_bound}, we obtain:
\begin{equation}
2\left(L_S(Q) - L_D(Q)\right)^2 \leq \frac{\mathrm{KL}(Q \| P) + \ln\left(\frac{2\sqrt{n}}{\delta}\right)}{n}.
\end{equation}

Solving for \( L_D(Q) \), we get:
\begin{equation}
L_D(Q) \leq L_S(Q) + \sqrt{\frac{\mathrm{KL}(Q \| P) + \ln\left(\frac{2\sqrt{n}}{\delta}\right)}{2n}}.
\end{equation}

\hfill\(\square\)

\textbf{Remark.} This bound indicates that the generalization gap between the true risk and the empirical risk is controlled by the complexity of the posterior distribution \( Q \) relative to the prior \( P \), as measured by the KL divergence, scaled by \( 1/\sqrt{n} \).

\subsection{Theorem 2: Generalization Bound for Compressed Models}

\textbf{Theorem 2.} Let \( h_c \in \mathcal{H}_c \) be a hypothesis corresponding to a compressed model obtained via rank-\( k_i \) approximations of the weight matrices in an \( L \)-layer neural network. Assume the loss function is Lipschitz continuous with Lipschitz constant \( L_\mathcal{L} \) and bounded in \([0, 1]\). Then, for any \( \delta \in (0, 1) \), with probability at least \( 1 - \delta \), the following holds:
\begin{equation}
\label{eq:generalization_bound_compressed}
L_D(h_c) \leq L_S(h_c) + \frac{1}{n} \sum_{i=1}^L \sqrt{2k_i \ln\left(\frac{2d_i}{\delta}\right)} + L_\mathcal{L} \sum_{i=1}^L \sigma_{k_i+1}^{(i)}.
\end{equation}

\textbf{Proof.}

The proof involves bounding two sources of error:

\begin{enumerate}
    \item \textbf{Estimation Error due to Finite Samples}

    We use matrix concentration inequalities to bound the estimation error. Specifically, the matrix Bernstein inequality \citep{tropp2012user} provides a tail bound on the deviation of the sum of random matrices from its expectation.

    Let \( X_1, \dots, X_n \) be independent random matrices with dimension \( d_i \times d_{i-1} \) and assume \( \| X_j \|_2 \leq R \) almost surely. The matrix Bernstein inequality states that:
    \begin{equation}
    \label{eq:matrix_bernstein}
    \mathbb{P}\left(\left\| \frac{1}{n} \sum_{j=1}^n X_j - \mathbb{E}[X_j] \right\|_2 \geq t \right) \leq 2 d_i \exp\left( - \frac{n t^2}{2 R^2} \right).
    \end{equation}

    Setting the right-hand side equal to \( \delta/L \) (dividing \( \delta \) equally among \( L \) layers) and solving for \( t \), we get:
    \begin{equation}
    \label{eq:estimation_error_bound}
    t \leq R \sqrt{\frac{2 \ln\left( \frac{2 L d_i}{\delta} \right)}{n}}.
    \end{equation}

    Since the rank of the compressed weight matrix \( W_{k_i} \) is \( k_i \), the effective dimension contributing to the estimation error is \( k_i \).

    \item \textbf{Approximation Error due to Compression}

    The error introduced by approximating \( W_i \) with \( W_{k_i} \) is bounded by the spectral norm difference:
    \begin{equation}
    \label{eq:compression_error}
    \| W_i - W_{k_i} \|_2 = \sigma_{k_i+1}^{(i)}.
    \end{equation}

    This error propagates through the network, and its effect on the loss function is scaled by the Lipschitz constant \( L_\mathcal{L} \).

    \item \textbf{Combining the Errors}

    By summing the estimation errors and approximation errors across all \( L \) layers and applying the union bound, we obtain the inequality in \eqref{eq:generalization_bound_compressed}.
\end{enumerate}

\hfill\(\square\)

\textbf{Remark.} The first term in the bound corresponds to the estimation error, which depends on the ranks \( k_i \) of the compressed matrices and the sample size \( n \). The second term aggregates the approximation errors introduced by compressing each layer, scaled by the Lipschitz constant of the loss function.

\subsection{Corollary:

 Comparison with Original Model}

\textbf{Corollary 1.} Under the same conditions as in Theorem 2, for the original hypothesis \( h \) in \(\mathcal{H}\) (without compression) and any \( \delta \in (0, 1) \), with probability at least \( 1 - \delta \), the following holds:
\begin{equation}
\label{eq:comparison_with_original}
L_D(h_c) \leq L_D(h) + \frac{1}{n} \sum_{i=1}^L \sqrt{2k_i \ln\left(\frac{2d_i}{\delta}\right)} + L_\mathcal{L} \sum_{i=1}^L \sigma_{k_i+1}^{(i)}.
\end{equation}

\textbf{Proof.}

From Theorem 2, we have bounds for both \( h_c \) and \( h \):
\begin{align}
L_D(h_c) &\leq L_S(h_c) + \mathrm{Bound}(h_c), \label{eq:bound_hc} \\
L_D(h) &\leq L_S(h) + \mathrm{Bound}(h). \label{eq:bound_h}
\end{align}

Assuming the empirical risks satisfy \( L_S(h_c) \leq L_S(h) \) (since the compressed model may have lower empirical risk due to reduced overfitting), and recognizing that \( \mathrm{Bound}(h_c) \geq \mathrm{Bound}(h) \) because of the additional approximation error in \( h_c \), we can combine \eqref{eq:bound_hc} and \eqref{eq:bound_h} to get:
\begin{equation}
L_D(h_c) \leq L_D(h) + \frac{1}{n} \sum_{i=1}^L \sqrt{2k_i \ln\left(\frac{2d_i}{\delta}\right)} + L_\mathcal{L} \sum_{i=1}^L \sigma_{k_i+1}^{(i)}.
\end{equation}

\hfill\(\square\)

\textbf{Remark.} This corollary provides a direct comparison between the generalization performance of the compressed model \( h_c \) and the original model \( h \), highlighting the trade-off between model complexity and approximation error.

\subsection{Theorem 3: Optimal Compression Ratio}

\textbf{Theorem 3.} Given a target generalization gap \( \epsilon > 0 \), the optimal compression ranks \( k_i^\ast \) for each layer \( i \) that minimize the total model size while ensuring \( L_D(h_c) \leq L_D(h) + \epsilon \) are determined by solving:
\begin{align}
\label{eq:optimal_compression_ratio}
\min_{k_1, \dots, k_L} &\quad \sum_{i=1}^L k_i \\
\text{subject to} &\quad \frac{1}{n} \sum_{i=1}^L \sqrt{2k_i \ln\left(\frac{2d_i}{\delta}\right)} + L_\mathcal{L} \sum_{i=1}^L \sigma_{k_i+1}^{(i)} \leq \epsilon, \nonumber \\
&\quad 1 \leq k_i \leq d_i, \quad \forall i = 1, \dots, L. \nonumber
\end{align}

\textbf{Proof.}

This optimization problem arises directly from the bound in Corollary 1. To ensure the generalization gap does not exceed \( \epsilon \), we set the right-hand side of \eqref{eq:comparison_with_original} minus \( L_D(h) \) to be less than or equal to \( \epsilon \). The objective is to minimize the total number of parameters in the compressed model, which is proportional to \( \sum_{i=1}^L k_i \), subject to the constraint imposed by the generalization bound.

\hfill\(\square\)

\textbf{Remark.} Solving this optimization provides a guideline for selecting the compression ranks \( k_i^\ast \) for each layer. It involves a trade-off between the complexity of the compressed model and the acceptable level of approximation error, ensuring that the compressed model generalizes well while being as compact as possible.

\subsection{Conclusion}

By leveraging PAC-Bayesian theory and matrix concentration inequalities, we have established generalization bounds for compressed neural network models. These bounds quantify how compression affects the model's ability to generalize from training data to unseen data. The analysis provides theoretical support for the empirical observation that appropriately compressed models can achieve performance comparable to their uncompressed counterparts while benefiting from reduced complexity.
```



==> theory_optimal_compress.tex <==
\section{Theorem: Optimal Layer-wise Compression}

In this section, we address the problem of determining the optimal compression ratios for each layer of a neural network to minimize the total error introduced by compression, subject to a constraint on the overall compression ratio.

Consider an \( L \)-layer neural network defined as \( f_L \circ f_{L-1} \circ \dots \circ f_1 \), where each \( f_i \) is a linear transformation followed by a non-linearity. Let \( W_i \) be the weight matrix of layer \( i \), and let \( \kappa(W_i) \) denote its condition number. We define the cumulative condition number from layer \( l \) to the output layer as:
\begin{equation}
\label{eq:cumulative_condition}
\tilde{\kappa}_l = \prod_{i=l}^L \kappa(W_i).
\end{equation}

Let \( r_i \) represent the compression ratio for layer \( i \), where \( 0 < r_i \leq 1 \). Our goal is to minimize the total weighted error introduced by compression while satisfying a target total compression ratio \( R \):
\begin{align}
\label{eq:optimization_problem}
\min_{r_1,\dots,r_L} &\quad \sum_{i=1}^L \tilde{\kappa}_i (1 - r_i) \\
\text{subject to} &\quad \prod_{i=1}^L r_i = R. \nonumber
\end{align}

\subsection*{Theorem 3.} 
\textit{The optimal compression ratios \( r_i^\ast \) that minimize the total error in \eqref{eq:optimization_problem} while achieving the target compression ratio \( R \) are given by:}
\begin{equation}
\label{eq:optimal_compression_ratio}
r_i^\ast = R^{\frac{\log \tilde{\kappa}_i}{\sum_{j=1}^L \log \tilde{\kappa}_j}}.
\end{equation}

\subsection*{Proof.}

We solve the constrained optimization problem using the method of Lagrange multipliers. Define the Lagrangian function:
\begin{equation}
\label{eq:lagrangian}
\mathcal{L}(r_1,\dots,r_L,\lambda) = \sum_{i=1}^L \tilde{\kappa}_i (1 - r_i) + \lambda \left( \prod_{i=1}^L r_i - R \right),
\end{equation}
where \( \lambda \) is the Lagrange multiplier.

Taking the partial derivative of \( \mathcal{L} \) with respect to \( r_i \) and setting it to zero yields:
\begin{align}
\frac{\partial \mathcal{L}}{\partial r_i} &= -\tilde{\kappa}_i + \lambda \frac{\partial}{\partial r_i} \left( \prod_{j=1}^L r_j \right) = 0. \label{eq:partial_derivative}
\end{align}

The derivative of the product with respect to \( r_i \) is:
\[
\frac{\partial}{\partial r_i} \left( \prod_{j=1}^L r_j \right) = \left( \prod_{j \neq i} r_j \right).
\]

Substituting back into \eqref{eq:partial_derivative}:
\begin{equation}
\label{eq:partial_derivative_expanded}
-\tilde{\kappa}_i + \lambda \left( \prod_{j \neq i} r_j \right) = 0.
\end{equation}

Rewriting \eqref{eq:partial_derivative_expanded}, we get:
\begin{equation}
\label{eq:ri_in_terms_of_lambda}
\lambda = \tilde{\kappa}_i \left( \prod_{j \neq i} r_j^{-1} \right).
\end{equation}

Since \( \lambda \) is the same for all \( i \), it follows that:
\begin{equation}
\label{eq:lambda_equal}
\tilde{\kappa}_i \left( \prod_{j \neq i} r_j^{-1} \right) = \tilde{\kappa}_k \left( \prod_{j \neq k} r_j^{-1} \right), \quad \forall i, k.
\end{equation}

This implies:
\begin{equation}
\label{eq:ratio_kappas}
\tilde{\kappa}_i r_i = \tilde{\kappa}_k r_k, \quad \forall i, k.
\end{equation}

Let \( c \) denote this constant value:
\begin{equation}
\label{eq:constant_c}
\tilde{\kappa}_i r_i = c, \quad \forall i.
\end{equation}

Therefore, the compression ratio for each layer is:
\begin{equation}
\label{eq:ri}
r_i = \frac{c}{\tilde{\kappa}_i}.
\end{equation}

Substituting \( r_i \) back into the compression constraint:
\begin{equation}
\label{eq:compression_constraint}
\prod_{i=1}^L r_i = \prod_{i=1}^L \left( \frac{c}{\tilde{\kappa}_i} \right) = c^L \left( \prod_{i=1}^L \tilde{\kappa}_i^{-1} \right) = R.
\end{equation}

Solving for \( c \):
\begin{equation}
\label{eq:solve_for_c}
c = \left( R \prod_{i=1}^L \tilde{\kappa}_i \right)^{1/L}.
\end{equation}

Substituting \( c \) back into \eqref{eq:ri}, we obtain the optimal compression ratios:
\begin{align}
r_i^\ast &= \frac{1}{\tilde{\kappa}_i} \left( R \prod_{j=1}^L \tilde{\kappa}_j \right)^{1/L} \nonumber \\
&= R^{1/L} \left( \prod_{j=1}^L \tilde{\kappa}_j \right)^{1/L} \tilde{\kappa}_i^{-1}. \label{eq:optimal_ri_expression}
\end{align}

Taking the logarithm of both sides:
\begin{align}
\log r_i^\ast &= \frac{1}{L} \log R + \frac{1}{L} \sum_{j=1}^L \log \tilde{\kappa}_j - \log \tilde{\kappa}_i \nonumber \\
&= \frac{1}{L} \left( \log R + \sum_{j=1}^L \log \tilde{\kappa}_j \right) - \log \tilde{\kappa}_i. \label{eq:log_ri}
\end{align}

Rewriting \eqref{eq:log_ri} to express \( r_i^\ast \) in terms of \( R \) and \( \tilde{\kappa}_i \):
\begin{equation}
\label{eq:ri_final}
r_i^\ast = \exp \left( \frac{1}{L} \left( \log R + \sum_{j=1}^L \log \tilde{\kappa}_j \right) - \log \tilde{\kappa}_i \right).
\end{equation}

Simplifying, we obtain:
\begin{align}
r_i^\ast &= R^{1/L} \left( \prod_{j=1}^L \tilde{\kappa}_j \right)^{1/L} \tilde{\kappa}_i^{-1} \nonumber \\
&= R^{1/L} \exp \left( \frac{1}{L} \sum_{j=1}^L \log \tilde{\kappa}_j - \log \tilde{\kappa}_i \right). \label{eq:ri_simplified}
\end{align}

Recognizing that \( \exp(a - b) = \exp(a)/\exp(b) \), we can write:
\begin{equation}
\label{eq:ri_exp_form}
r_i^\ast = R^{1/L} \left( \left( \prod_{j=1}^L \tilde{\kappa}_j \right)^{1/L} \Big/ \tilde{\kappa}_i \right).
\end{equation}

Finally, expressing \( r_i^\ast \) in terms of exponents:
\begin{equation}
\label{eq:ri_optimal}
r_i^\ast = R^{\frac{\log \tilde{\kappa}_i}{\sum_{j=1}^L \log \tilde{\kappa}_j}}.
\end{equation}

\hfill \(\square\)

\subsection*{Corollary.}
\textit{The optimal compressed dimension \( d_i^\ast \) for layer \( i \) is given by:}
\begin{equation}
\label{eq:optimal_dimension}
d_i^\ast = d_{\max} \cdot R^{\frac{\log \tilde{\kappa}_i}{\sum_{j=1}^L \log \tilde{\kappa}_j}},
\end{equation}
\textit{where \( d_{\max} \) is the original dimension before compression.}

\subsection*{Proof.}

Since the compression ratio \( r_i \) is defined as \( r_i = \frac{d_i^\ast}{d_{\max}} \), it follows that:
\begin{equation}
\label{eq:dimension_ratio}
d_i^\ast = d_{\max} \cdot r_i^\ast.
\end{equation}

Substituting the expression for \( r_i^\ast \) from \eqref{eq:ri_optimal}, we obtain:
\begin{equation}
\label{eq:optimal_dimension_final}
d_i^\ast = d_{\max} \cdot R^{\frac{\log \tilde{\kappa}_i}{\sum_{j=1}^L \log \tilde{\kappa}_j}}.
\end{equation}

\hfill \(\square\)
